Nowcasting Growth using Google Trends Data: A Bayesian Structural Time Series Model

This paper investigates the benefits of internet search data in the form of Google Trends for nowcasting real U.S. GDP growth in real time through the lens of mixed frequency Bayesian Structural Time Series (BSTS) models. We augment and enhance both model and methodology to make these better amenable to nowcasting with large number of potential covariates. Specifically, we allow shrinking state variances towards zero to avoid overfitting, extend the SSVS (spike and slab variable selection) prior to the more flexible normal-inverse-gamma prior which stays agnostic about the underlying model size, as well as adapt the horseshoe prior to the BSTS. The application to nowcasting GDP growth as well as a simulation study demonstrate that the horseshoe prior BSTS improves markedly upon the SSVS and the original BSTS model with the largest gains in dense data-generating-processes. Our application also shows that a large dimensional set of search terms is able to improve nowcasts early in a specific quarter before other macroeconomic data become available. Search terms with high inclusion probability have good economic interpretation, reflecting leading signals of economic anxiety and wealth effects.

==> Chapters/Methodology.tex <==
% 1. Non-Centred State Space
\subsection{Non-Centred State Space} \label{subsec:statespace}
The original state space formulation of \citet{scott2014predicting} collects states $\tau_t$, $\alpha_t$ and $\delta_t$ in (\ref{equ:bsts}) and estimates them jointly via the forward
filtering backward sampling (FFBS) algorithm of \citet{durbin2002simple} based on the Kalman filter. While very popular, the recursive structure of the algorithm is costly in terms of computation, but more importantly, relies on independent Normal-Inverse Gamma (N-IG) priors for the states and state variances which \citet{fruhwirth2010stochastic} show can lead to overfitting state spaces and therefore imprecise forecasts. This is due to the fact that in state space models, the state variances determine whether a state process is fixed or time varying (see equation (\ref{equ:bsts})). Instead, \citet{fruhwirth2010stochastic} propose a non-centred representation of the state space which dissects the dynamics into a non-time varying and a time varying component, where the former models the state standard deviation directly in the observation equation. A normal prior on the state standard deviation can be shown to imply a Gamma prior on the state variance which allows for far more mass on 0, therefore applying more shrinkage. 

Taking (\ref{equ:bsts}) as our centred state space (and ignoring $\mathbf{X}$ for now), we re-write it equivalently as:
\begin{equation} \label{eq:non-centred1}
    y_t = \tau_0 + \sigma_{\tau}\tilde{\tau}_t + t\alpha_0 + \sigma_{\alpha}\sum_{s=1}^t\tilde{\alpha}_t + \epsilon_t, \; \epsilon_t \sim N(0,\sigma^2)
\end{equation}
where
\begin{equation} \label{eq:non-centred2}
    \begin{split}
        \tilde{\tau}_t & = \tilde{\tau}_{t-1} + \tilde{u}^{\tau}_t, \tilde{u}^{\tau}_t \sim N(0,1) \\
        \tilde{\alpha}_t & = \tilde{\alpha}_{t-1} + \tilde{u}^{\alpha}_t, \tilde{u}^{\alpha}_t \sim N(0,1)
    \end{split}
\end{equation} 
with starting values $\tilde{\tau}_0 = \tilde{\alpha}_0 = 0$. To see that (\ref{eq:non-centred1}) and (\ref{eq:non-centred2}) is equivalent to (\ref{equ:bsts}), let:
\begin{equation}
    \begin{split}
        \alpha_t & = \alpha_0 + \sigma_{\alpha}\tilde{\alpha}_t \\
        \tau_t & = \tau_0 + \sigma_{\tau}\tilde{\tau}_t + t\alpha_0 + \sigma_{\alpha}\sum_{s=1}^t\alpha_s 
    \end{split}
\end{equation} \label{eq:non-centred3}
Hence, by setting $y_t = \tau_t +\epsilon_t$, it is clear that
\begin{equation}
    \begin{split}
        \alpha_t - \alpha_{t-1} & = \sigma{\alpha}(\tilde{\alpha}_t - \tilde{\alpha}_{t-1}) \\
        & = \sigma_{\alpha} + \tilde{u}^{\alpha}_t \\
        \tau_t - \tau_{t-1} & = \alpha_0 + \sigma_{\alpha}\tilde{\alpha}_t + \sigma_{\tau}(\tilde{\tau}_t - \tilde{\tau}_{t-1}) \\
        & = \alpha + \sigma_{\tau} + \tilde{u}^{\tau}_t
    \end{split}
\end{equation}
which recovers (\ref{equ:bsts}). Since $\sigma_{\tau,\alpha}$ are allowed to have support on the real line, they are not identified in multiplication with the states: the likelihood is invariant to signs of $\sigma_{\alpha}$ and $\sigma_{\tau}$. Consequently, mixing of the posterior state standard deviations can be poor and their distributions are likely to be bi-modal \citep{fruhwirth2010stochastic}. This issue is addressed by randomly permuting signs in the Gibbs sampler as explained below. Similar to \citet{fruhwirth2010stochastic}, we assume normal priors centred at 0 for $\sigma_i: \sigma_i \sim N(0,V_i)$ $\forall i \in \{\tau,\alpha\}$. 

Collecting all state space parameters in $\theta = (\tau_0,\alpha_0,\sigma_{\tau},\sigma_{\alpha})$, we assume an independent multivariate normal prior with diagonal covariance matrix:
\begin{equation}
    \theta \sim N(\theta_0,V_{\theta}).
\end{equation}
While the state processes $\{\tilde{\tau},\tilde{\alpha}\}^T_{t=1}$ can be estimated by any state space algorithm, we opt for the precision sampler method of \citet{chan2017notes} as outlined in Appendix (\ref{subsec:estimation}) . In contrast to FFSB type algorithms, it samples the states without recursive estimation which speeds up computation significantly. 

% 2: SSVS Prior
\subsection{SSVS Prior}
Variable selection in the BSTS model of \citet{scott2014predicting} is done via a two component conjugate spike-and-slab prior which utilises a variant of Zeller’s g-prior and fixed expected model size. While computationally fast due to conjugacy, many high-dimensional problems benefit from prior independence \citep{moran2018variance} and a fully hierarchical formulation to let the data decide on the most likely value of the parameters \citep{ishwaran2005spike}. 

Therefore, we follow \citet{ishwaran2005spike}'s extension to the SSVS prior, the Normal-Inverse-Gamma prior:
\begin{equation} \label{eq:nigprior}
    \begin{split}
    \beta_j|\gamma_j,\delta_j^2 & \sim \gamma_jN(0,\delta_j^2) + (1-\gamma_j)N(0,c\times\delta_j^2) \\
        \delta_j^2 & \sim Gamma(a_1.a_2) \\
        \gamma_j & \sim Bernoulli(\pi_0) \\
        \pi_0 & \sim Beta(b_1,b_2)
    \end{split}
\end{equation} 
where $j \in (1,\cdots,K)$. The intuition remains the same as compared to the spike-and-slab prior of \citet{scott2014predicting} in that the covariate's effect is modeled by a mixture of normals where it is either shrunk to close to zero via a narrow distribution around zero (the spike component) or estimated freely though a relatively diffuse normal distribution (the slab component). Sorting into each component is handled through an indicator variable, $\gamma_j$, and the hyperparameter c is chosen to be a very small number, thereby forcing shrinkage of noise variables to close to zero. While in the original BSTS model, the indicator variable, $\gamma_j$, depends on a fixed prior $\pi_0$ which governs the prior inclusion probability of a variable, (\ref{eq:nigprior}) allows for it to be estimated from the data through another level of hierarchy. We set $b_1=b_2=1$, which effectively assumes that any expected model size is a priori possible and thus allows for sparse but also dense model solutions as recommended by \citep{giannone2017economic}. Finally, the prior variance $\delta^2_j$ is also allowed to be hierarchical. Posteriors are standard and described in the Appendix (\ref{subsec:posteriors}). The posterior of $\gamma_j$ is of special interest to the analyst as it gives a data informed measure of importance of a variable. Namely,  $p(\gamma|y)$ can be interpreted as the posterior inclusion probability of a variable. \\
% 3. Horseshoe Prior
\subsection{Horseshoe Prior}
Like many recently popularised shrinkage priors, the horseshoe prior belongs to the broader class of global-local priors which take the following general form:
\begin{equation}
\begin{split}
     \beta_j | \lambda_j^2, \nu^2, \sigma^2 & \sim N(0,\lambda_j^2\nu^2\sigma^2), j \in (1,\cdots, K) \\
    \lambda_j & \sim \pi(\lambda_j)d\lambda_j, j \in (1,\cdots, K) \\
    \nu & \sim \pi(\nu)d\nu
    \end{split}
\end{equation} \label{eq:glpriors}
The idea of this family of priors is that the global scale $\nu^2$ controls the overall shrinkage applied to the regression, while the local scale $\lambda^2_j$ allows for the local possibility of regressors to escape shrinkage if they have large effects on the response. A variety of global local shrinkage priors have been proposed (\cite{polson2010shrink}), but here we focus on arguably the most popular, the horseshoe prior of \cite{carvalho2010horseshoe} which employs two half Cauchy distributions for $\nu$ and $\lambda_j$:
\begin{equation}  \label{prior5}
 \begin{split}
     \lambda_j & \sim C_+(0,1) \\
     \nu & \sim C_+(0,1) 
 \end{split}
 \end{equation} 
These two fat tailed priors imply a shrinkage profile that has the spike-and-slab prior in its limit and therefore offers a continuous approximation to the SSVS \citep{piironen2017sparsity}. Due to its special connection to frequentist shrinkage priors \citep{polson2010shrink}, it offers not only good finite sample performance but also favourable asymptotic behaviour compared to competing global priors \citep{bhadra2019lasso}. Posteriors are described in the appendix (\ref{subsec:posteriors}).

% 4. SAVS algorithm
\subsection{SAVS Algorithm}
Although the horseshoe prior will shrink noise variables towards zero, the importance of a variable for nowcasts may not be immediately clear from posterior summary statistics of the coefficients, especially when the posterior is multi-modal. To aid interpretability and simultaneously preserve predictive ability, we employ the SAVS algorithm of \cite{ray2018signal} to the posterior coefficients on a draw-by-draw basis. The algorithm uses a useful heuristic, inspired by frequentist lasso estimation, to threshold posterior regression coefficients to zero:
\begin{equation}\label{eq:savs1}
    \phi_j = sign(\hat{\beta}_j)||X_j||^{-2}max(|\hat{\beta}_j|\;||X_j||-\kappa_j,0),
\end{equation}
where $X_j = (x_{j1},\cdots,x_{jT})'$ is the $j^{th}$ column of the regressor matrix X, sign(x) returns the sign of x and $\hat{\beta}$ represents a draw from the regression posterior. The parameter $\kappa_j$ in (\ref{eq:savs1}) acts as a threshold for each coefficient akin to the penalty parameter in lasso regression which can be selected via cross-validation. \citet{ray2018signal} propose
\begin{equation}\label{eq:savs2}
    \kappa_j = \frac{1}{|\beta_j|^2},
\end{equation}
which ranks the coefficients inverse-squared proportionally and provides good performance compared to alternate penalty levels \citep{ray2018signal,huber2019inducing}. To see the similarity to lasso style regularisation, the solution to (\ref{eq:savs1}) can be obtained by the following minimisation problem which is closely related to the adaptive lasso \citep{zou2006adaptive}: 
\begin{equation}\label{eq:savs3}
    \overline{\phi} = \underset{\phi}{\mathrm{argmin}}\bigg\{\frac{1}{2}||X\hat{\beta}-X\phi|| + \sum^K_{j=1}\kappa_j|\phi_j|\bigg\}.
\end{equation}
Here, $\overline{\phi}$ is the sparsified regression vector. Analogous to the SSVS posterior, the relative frequency of non-zero entries in the posterior coefficient vector can be interpreted as posterior inclusion probabilities. Together, integrating over the uncertainty of the parameters to obtain the predictive distribution $p(\tilde{y}|y)$, we receive something similar to a Bayesian Model Averaged (BMA) posterior \citep{koop2019macroeconomic}.

% 5. Sampling Algorithm
\subsection{Sampling Algorithm}
With the conditional posteriors at hand (see Appendix \ref{subsec:posteriors}), we sample states as well as regression parameters with the following Gibbs sampler:
\begin{enumerate} \label{gibbssampler}
    \item Sample $(\tilde{\tau},\tilde{\alpha}|y, \theta, \beta,\sigma^2_y)$
    \item Sample $(\theta|y,\beta,\tilde{\tau},\tilde{\alpha},\sigma^2_y)$
    \item Randomly permute signs of $(\tilde{\tau},\tilde{\alpha})$ and $(\sigma_{\tau},\sigma_{\alpha})$
    \item Sample $(\beta|y,\theta,\tilde{\tau},\tilde{\alpha},\sigma^2_y)$
    \item Sample $(\sigma^2_y|y,\tilde{\tau},\tilde{\alpha},\sigma^2_y)$
\end{enumerate}

As mentioned in Section \ref{subsec:statespace}, states are sampled in a non-recursive fashion which exploits sparse matrix computation and precision sampling. The exact sampling algorithm is given in Appendix  \ref{subsec:estimation}. As discussed in Section \ref{subsec:statespace}, after sampling $\theta$ in step 2, we randomly permute signs of $(\tilde{\tau},\tilde{\alpha}),(\sigma_{\tau},\sigma_{\alpha})$ to aid mixing. Step 4 of the sampler will depend on the prior and its respective hyperpriors. While the posterior sampling scheme for the SSVS is standard, we use the efficient posterior sampler of \citet{bhattacharya2016fast} to sample the regression coefficients of the horseshoe prior. Compared to Cholesky based sampling as used for the SSVS, computation speed is markedly improved; see Appendix  \ref{subsubsec:hs}. Note that in step 4, we perform SAVS sparsification via (\ref{eq:savs1}) on an iteration basis. 

==> backup.tex <==

\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
 $p$ &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
HS-BQR & 0.217 & 0.247 & 0.142 & 0.204
 & 0.176 & 0.18 \\
LBQR &  0.364** & 0.056 & 0.017 & 0.046 & 0.023 & 0.015 \\
BQRENET & 0.426*** & 0.054 & 0.052 & 0.12 & 0.026 & 0.01 \\
BALQR & 0.433*** & 0.001 & 0 & 0.033 & 0.019 & 0.078 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for 2-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantile levels.}
\label{tab:fitofestimates}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
 $p$ &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
HS-BQR & 0.247 & 0.158 & 0.117 & 0.147
 & 0.101 & 0.188 \\
LBQR &  0.333** & 0.003 & 0.006 & 0.019 & 0.024 & 0.064 \\
BQRENET & 0.402*** & 0.043 & 0.058 & 0.103 & 0.067 & 0.011 \\
BALQR & 0.491*** & 0.007 & 0.002 & 0.008 & 0.058 & 0.076 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for 3-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantile levels.}
\label{tab:fitofestimates}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
 $p$ &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
HS-BQR & 0.193 & 0.296 & 0.13 & 0.132
 & 0.111 & 0.071 \\
LBQR &  0.398** & 0.015 & 0.014 & 0.051 & 0.008 & 0.01 \\
BQRENET & 0.370** & 0.023 & 0.01 & 0.063 & 0.008 & 0.001 \\
BALQR & 0.446*** & 0.052 & 0 & 0.017 & 0.035 & 0.088 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for 4-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantile levels.}
\label{tab:fitofestimates}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{rccccc}
\hline
 \multicolumn{5}{c}{Average Log-Scores} \\
  & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
HS-BQR & 3.432 & 3.282 & 3.472
 & 3.534 \\
LBQR & 3.235 & 3.294 & 3.396 & 3.431 \\
BQRENET & 2.999 & 3.369 & 3.426 & 3.430 \\
BALQR & 1.839 & 2.069 & 2.154 & 2.133 \\
SPF & 3.083 & 3.276 & 3.285 & 3.185 \\
\hline
\end{tabular}
\caption{Average log scores of the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Density is approximated by a normal kernel of the 19 forecasted quantiles.}
\label{tab:logscores}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{rccccc}
\hline
 \multicolumn{5}{c}{Median Quantile Forecasts} \\
  & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
HS-BQR & 0.006 & 0.004 & 0.004 & 0.004 \\
LBQR & 0.010*** & 0.012*** & 0.008*** & 0.008*** \\
BQRENET & 0.009*** & 0.007*** & 0.007*** & 0.008*** \\
BALQR & 0.015*** & 0.012*** & 0.010*** & 0.007*** \\
SPF & 0.005*** & 0.004*** & 0.004*** & 0.004*** \\
\hline
\end{tabular}
\caption{Mean-squared-forecast-errors based on the median quantiles for the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Stars indicate statistical difference to the HSBQR median forecasts based on the Diebold-Mariano test (1998) at 10\%, 5\% and 1\% significance respectively.}
\label{tab:MSFE}
\end{table}

% MANY ROWS 
\begin{table}[]
\centering
\begin{tabular}{rccccc}
\hline
  & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
 \multicolumn{5}{c}{Average Log-Scores} \\
 \hline
HS-BQR & 3.432 & 3.282 & 3.472
 & 3.534 \\
LBQR & 3.235 & 3.294 & 3.396 & 3.431 \\
BQRENET & 2.999 & 3.369 & 3.426 & 3.430 \\
BALQR & 1.839 & 2.069 & 2.154 & 2.133 \\
SPF & 3.083 & 3.276 & 3.285 & 3.185 \\
\hline
 \multicolumn{5}{c}{Median Quantile Forecasts} \\
 \hline
HS-BQR & 0.006 & 0.004 & 0.004 & 0.004 \\
LBQR & 0.010*** & 0.012*** & 0.008*** & 0.008*** \\
BQRENET & 0.009*** & 0.007*** & 0.007*** & 0.008*** \\
BALQR & 0.015*** & 0.012*** & 0.010*** & 0.007*** \\
SPF & 0.005*** & 0.004*** & 0.004*** & 0.004*** \\
\hline
\end{tabular}
\caption{Average log scores and the mean-squared-forecast errors of the median of the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Density for the log scores is approximated by a normal kernel of the 19 forecasted quantiles. Stars indicate statistical difference to the HSBQR median forecasts based on the Diebold-Mariano test (1998) at 10\%, 5\% and 1\% significance respectively.}
\label{tab:logscoresandMSFE}
\end{table}

%MANY COLUMNS
\begin{table}
\centering
\begin{tabular}{r|cccc|cccc}
\hline
 & \multicolumn{4}{c|}{Average Log-Scores} & \multicolumn{4}{c}{Median Quantile Forecasts}\\
  & h=1 & h=2 & h=3 & h=4 & h=1 & h=2 & h=3 & h=4 \\
 \hline
 \hline
HS-BQR & 3.432 & 3.282 & 3.472 & 3.534 & 0.006 & 0.004 & 0.004 & 0.004 \\
LBQR & 3.235 & 3.294 & 3.396 & 3.431 & 0.010*** & 0.012*** & 0.008*** & 0.008*** \\
BQRENET & 2.999 & 3.369 & 3.426 & 3.430 & 0.009*** & 0.007*** & 0.007*** & 0.008*** \\
BALQR & 1.839 & 2.069 & 2.154 & 2.133 & 0.015*** & 0.012*** & 0.010*** & 0.007*** \\
SPF & 3.083 & 3.276 & 3.285 & 3.185 & 0.005*** & 0.004*** & 0.004*** & 0.004***  \\
\hline
\end{tabular}
\caption{Average log scores and Mean-squared-forecast-errors on the median of the different estimators for 1-,2-,3- and 4-step-ahead quantile forecasts. Density is approximated by a normal kernel of the 19 forecasted quantiles. For the MSFE stars indicate statistical difference to the HSBQR median forecasts based on the Diebold-Mariano test (1998) at 10\%, 5\% and 1\% significance respectively.}
\label{tab:logscoresandMSFE}
\end{table}

%LONG TABLE
\begin{table}[]
\centering
\begin{tabular}{r|c|ccccc}
\hline
 & KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
  &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
 \multicolumn{7}{c}{\textit{1-step ahead}}\\
 \hline
HS-BQR & 0.195 & 0.256 & 0.13 & 0.102 & 0.15 & 0.234 \\
LBQR & 0.382*** & 0.049 & 0.083 & 0.028 & 0.031 & 0.067 \\
BQRENET & 0.396*** & 0.048 & 0.11 & 0.063 & 0.041 & 0.001 \\
BALQR & 0.443*** & 0.11 & 0.025 & 0 & 0.001 & 0.039 \\
 \hline
 \multicolumn{7}{c}{\textit{2-step ahead}}\\
 \hline
HS-BQR & 0.217 & 0.247 & 0.142 & 0.204 & 0.176 & 0.18 \\
LBQR &  0.364** & 0.056 & 0.017 & 0.046 & 0.023 & 0.015 \\
BQRENET & 0.426*** & 0.054 & 0.052 & 0.12 & 0.026 & 0.01 \\
BALQR & 0.433*** & 0.001 & 0 & 0.033 & 0.019 & 0.078 \\
 \hline
 \multicolumn{7}{c}{\textit{3-step ahead}}\\
 \hline
HS-BQR & 0.247 & 0.158 & 0.117 & 0.147 & 0.101 & 0.188 \\
LBQR &  0.333** & 0.003 & 0.006 & 0.019 & 0.024 & 0.064 \\
BQRENET & 0.402*** & 0.043 & 0.058 & 0.103 & 0.067 & 0.011 \\
BALQR & 0.491*** & 0.007 & 0.002 & 0.008 & 0.058 & 0.076 \\
 \hline
 \multicolumn{7}{c}{\textit{4-step ahead}}\\
 \hline
HS-BQR & 0.193 & 0.296 & 0.13 & 0.132 & 0.111 & 0.071 \\
LBQR &  0.398** & 0.015 & 0.014 & 0.051 & 0.008 & 0.01 \\
BQRENET & 0.370** & 0.023 & 0.01 & 0.063 & 0.008 & 0.001 \\
BALQR & 0.446*** & 0.052 & 0 & 0.017 & 0.035 & 0.088 \\
\hline
\end{tabular}
\caption{Performance of the different estimators for h-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantiles}
\label{tab:fitofestimates}
\end{table}

%WIDE TABLE
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{r|c|ccccc|c|ccccc}
\hline
 & KS & \multicolumn{5}{c|}{Pseudo-$R^2$}& KS & \multicolumn{5}{c}{Pseudo-$R^2$} \\
  &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 &  & 0.05 & 0.25 & 0.5 & 0.75 & 0.95 \\
 \hline
 \hline
 & \multicolumn{6}{c|}{\textit{1-step ahead}} & \multicolumn{6}{c}{\textit{2-step ahead}}\\
 \hline
HS-BQR & 0.195 & 0.256 & 0.13 & 0.102 & 0.15 & 0.234 & 0.217 & 0.247 & 0.142 & 0.204 & 0.176 & 0.18 \\
LBQR & 0.382*** & 0.049 & 0.083 & 0.028 & 0.031 & 0.067 &  0.364** & 0.056 & 0.017 & 0.046 & 0.023 & 0.015 \\
BQRENET & 0.396*** & 0.048 & 0.11 & 0.063 & 0.041 & 0.001 & 0.426*** & 0.054 & 0.052 & 0.12 & 0.026 & 0.01 \\
BALQR & 0.443*** & 0.11 & 0.025 & 0 & 0.001 & 0.039 & 0.433*** & 0.001 & 0 & 0.033 & 0.019 & 0.078 \\
 \hline
 & \multicolumn{6}{c|}{\textit{3-step ahead}} & \multicolumn{6}{c}{\textit{4-step ahead}}\\
 \hline
HS-BQR & 0.247 & 0.158 & 0.117 & 0.147 & 0.101 & 0.188 & 0.193 & 0.296 & 0.13 & 0.132 & 0.111 & 0.071 \\
LBQR &  0.333** & 0.003 & 0.006 & 0.019 & 0.024 & 0.064 &  0.398** & 0.015 & 0.014 & 0.051 & 0.008 & 0.01 \\
BQRENET & 0.402*** & 0.043 & 0.058 & 0.103 & 0.067 & 0.011 & 0.370** & 0.023 & 0.01 & 0.063 & 0.008 & 0.001 \\
BALQR & 0.491*** & 0.007 & 0.002 & 0.008 & 0.058 & 0.076 & 0.446*** & 0.052 & 0 & 0.017 & 0.035 & 0.088 \\
 \hline
\end{tabular}}
\caption{Performance of the different estimators for h-step-ahead quantile forecasts. The first column, KS, reports the Kolmogorov-Smirnov test for equality to a uniform CDF with critical values of 0.374. 0.312 and 0.28 for the 1\%, 5\% and 10\% critical values respectively (indicated by ***,** and *). Pseudo-$R^2$ are shown the right most panel for a set of 5 chosen quantiles.}
\label{tab:fitofestimates}
\end{table}
